Interaction and Identification of the Meson-Baryon molecules

The challenges with the molecular model of the multiquark systems are the identification of the hadronic molecules and the interaction between two color neutral hadrons. We study the di-hadronic molecular systems with proposed interaction potential as s-wave one boson exchange potential along with Screen Yukawa-like potential, and arrived with the proposal that within hadronic molecule the two color neutral hadrons experience the dipole-like interaction. The present study is the continuation of our previous study \cite{arxiv-Rathaud-penta}. With the proposed interaction potential, the mass spectra of $\Sigma_{s}K^{*}$, $\Sigma_{c}K^{*}$, $\Sigma_{b}K^{*}$, $\Sigma_{s}D^{*}$, $\Sigma_{c}D^{*}$, $\Sigma_{b}D^{*}$, $\Sigma_{s}B^{*}$, $\Sigma_{c}B^{*}$, $\Sigma_{b}B^{*}$, $\Xi_{s}K^{*}$, $\Xi_{c}K^{*}$, $\Xi_{b}K^{*}$, $\Xi_{s}D^{*}$, $\Xi_{c}D^{*}$, $\Xi_{b}D^{*}$, $\Xi_{s}B^{*}$, $\Xi_{c}B^{*}$, $\Xi_{b}B^{*}$ meson-baryon molecules are predicted. The Weinberg compositeness theorem which provides clue for the compositeness of the state is used for determination of the scattering length and effective range. The present study predict $P_{c}(4450)$ pentaquark sate as $\Sigma_{c}D^{*}$ molecule with $I(J^{P})=\frac{1}{2}(\frac{3}{2}^{-})$. The formalism also predicts some very interesting open as well as hidden flavour near threshold molecular pentaquark states.

==> fig/SigmaPlot <==
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-NET-P1.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-NET-P2.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-NET-P3.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-NET-P4.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-NET-P5.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-NET-P6.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-NET-P7.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-NET-P8.pdf}

\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-NET-P9.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-NET-P10.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-NET-P11.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-NET-P12.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-NET-P13.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-NET-P14.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-NET-P15.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-NET-P16.pdf}

\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-NET-P17.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-NET-P18.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-NET-P19.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-NET-P20.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-NET-P21.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-NET-P22.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-NET-P23.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-NET-P24.pdf}

\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-OBE-P1.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-OBE-P2.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-OBE-P3.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-OBE-P4.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-OBE-P5.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-OBE-P6.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-OBE-P7.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-OBE-P8.pdf}

\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-OBE-P9.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-OBE-P10.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-OBE-P11.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-OBE-P12.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-OBE-P13.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-OBE-P14.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-OBE-P15.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-OBE-P16.pdf}

\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-OBE-P17.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-OBE-P18.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-OBE-P19.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-OBE-P20.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-OBE-P21.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-OBE-P22.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-OBE-P23.pdf}
\includegraphics[scale=0.45]{fig/SigmaS-D*-NN-OBE-P24.pdf}






